Fewer Tokens, Better Action: GPT-6 Astra Robot Agents with 14% Higher Success Rate but 65% Fewer Tokens

Vision-language model (VLM) agents can control robots through visual feedback and action primitives, but repeated LLM calls and redundant observations incur substantial token overhead. We introduce PyRUA-Lean, an interactive code-execution framework in which the agent composes robot primitives, including vision-language-action (VLA) policies, into Python cells that check and retry locally and return only the images and state they request. Across 700 simulated task instances from LIBERO-PRO, RoboTwin 2.0, and RoboCasa365, it raises success from 63.1% to 71.7% over tool calling with the same GPT-6 Astra planner and primitives, using 49% fewer LLM calls and 65% fewer input tokens on jointly solved instances. On RoboDojo, without any VLA policy or privileged information, it reaches 51.6% average success rate (Score 58.2), 19.4 points above the top entry of the public leaderboard. Based on the PyRUA-Lean framework, we train PyRUA-Lean Coder v0.1-4B, an open 4B model, with GRPO on 45 LIBERO-PRO instances; it improves from 18.8% to 44.1% on unseen task instances, surpassing the Qwen3.5-27B base model.

==> generated/v2_values.tex <==
% generated by scripts/v2_numbers.py from the RoboDojo and card-protocol result files -- do not edit
\makeatletter
\expandafter\def\csname pv@CD_B27_BEH_BUDGET\endcsname{35.0}
\expandafter\def\csname pv@CD_B27_BEH_IMG\endcsname{22.5}
\expandafter\def\csname pv@CD_B27_BEH_OVERFLOW\endcsname{31.0}
\expandafter\def\csname pv@CD_B27_UNSEEN\endcsname{29.2}
\expandafter\def\csname pv@CD_B4_BEH_BUDGET\endcsname{52.7}
\expandafter\def\csname pv@CD_B4_BEH_IMG\endcsname{19.3}
\expandafter\def\csname pv@CD_B4_BEH_LLMCALLS\endcsname{9.4}
\expandafter\def\csname pv@CD_B4_BEH_MULTI\endcsname{89}
\expandafter\def\csname pv@CD_B4_BEH_OVERFLOW\endcsname{19.2}
\expandafter\def\csname pv@CD_B4_BEH_PER_CALL\endcsname{9.0}
\expandafter\def\csname pv@CD_B4_HELD\endcsname{13.5}
\expandafter\def\csname pv@CD_B4_RCA\endcsname{52.2}
\expandafter\def\csname pv@CD_B4_RCC\endcsname{12.5}
\expandafter\def\csname pv@CD_B4_RT\endcsname{14.0}
\expandafter\def\csname pv@CD_B4_TRAIN\endcsname{37.8}
\expandafter\def\csname pv@CD_B4_UNSEEN\endcsname{18.8}
\expandafter\def\csname pv@CD_BEH_LIMIT_NOTE\endcsname{\ An episode that reached a limit with its task already complete counts as solved (three episodes of Qwen3.5-4B and one episode of Qwen3.5-27B).}
\expandafter\def\csname pv@CD_BEH_NOTE\endcsname{}
\expandafter\def\csname pv@CD_C4_ALL\endcsname{45.9}
\expandafter\def\csname pv@CD_C4_BEH_BUDGET\endcsname{10.5}
\expandafter\def\csname pv@CD_C4_BEH_GAVEUP\endcsname{25.2}
\expandafter\def\csname pv@CD_C4_BEH_IMG\endcsname{0.8}
\expandafter\def\csname pv@CD_C4_BEH_OVERFLOW\endcsname{3.4}
\expandafter\def\csname pv@CD_C4_BEH_TIMEOUT\endcsname{16.8}
\expandafter\def\csname pv@CD_C4_HELD\endcsname{37.4}
\expandafter\def\csname pv@CD_C4_RCA\endcsname{76.7}
\expandafter\def\csname pv@CD_C4_RCC\endcsname{19.4}
\expandafter\def\csname pv@CD_C4_RT\endcsname{52.4}
\expandafter\def\csname pv@CD_C4_TRAIN\endcsname{71.1}
\expandafter\def\csname pv@CD_C4_UNSEEN\endcsname{44.1}
\expandafter\def\csname pv@CD_COUNT_NOTE\endcsname{}
\expandafter\def\csname pv@CD_FORCED_NOTE\endcsname{}
\expandafter\def\csname pv@CD_GPT_ALL\endcsname{71.7}
\expandafter\def\csname pv@CD_STAR_NOTE\endcsname{}
\expandafter\def\csname pv@CD_TR_FIRST\endcsname{0.30}
\expandafter\def\csname pv@CD_TR_LAST5\endcsname{0.70}
\expandafter\def\csname pv@RDD_EPISODES\endcsname{6{,}300}
\expandafter\def\csname pv@RDD_LLM_MEAN\endcsname{23.9}
\expandafter\def\csname pv@RDD_SCORE\endcsname{58.8}
\expandafter\def\csname pv@RDD_SEED_PHRASE\endcsname{three evaluation seeds}
\expandafter\def\csname pv@RDD_SEED_SRS\endcsname{52.4\%, 53.2\% and 53.1\%}
\expandafter\def\csname pv@RDD_SR\endcsname{52.9}
\expandafter\def\csname pv@RDD_SR_SD\endcsname{0.35}
\expandafter\def\csname pv@RDD_USD_EPISODE\endcsname{2.2}
\expandafter\def\csname pv@RDD_USD_PROTOCOL_K\endcsname{14}
\expandafter\def\csname pv@RDX_D_SCORE\endcsname{58.6}
\expandafter\def\csname pv@RDX_D_SR\endcsname{52.4}
\expandafter\def\csname pv@RDX_MAXDIFF_D\endcsname{41.0}
\expandafter\def\csname pv@RDX_MAXDIFF_DIM\endcsname{Precision}
\expandafter\def\csname pv@RDX_MAXDIFF_RGB\endcsname{37.3}
\expandafter\def\csname pv@RDX_RGB_SCORE\endcsname{58.2}
\expandafter\def\csname pv@RDX_RGB_SR\endcsname{51.6}
\expandafter\def\csname pv@RDX_SCOPE\endcsname{the seed that both configurations ran}
\expandafter\def\csname pv@RD_ABOVE_ASTRA_N\endcsname{34}
\expandafter\def\csname pv@RD_ASTRA_LONG_SR\endcsname{8.3}
\expandafter\def\csname pv@RD_ASTRA_PREC_SR\endcsname{4.0}
\expandafter\def\csname pv@RD_ASTRA_SR\endcsname{22.5}
\expandafter\def\csname pv@RD_BELOW_ASTRA_N\endcsname{2}
\expandafter\def\csname pv@RD_BOARD_DATE\endcsname{October 9, 2026}
\expandafter\def\csname pv@RD_BOARD_N\endcsname{33}
\expandafter\def\csname pv@RD_BOARD_SHOWN_PHRASE\endcsname{the first ten entries (the tenth is GPT-6 Astra with direct control)}
\expandafter\def\csname pv@RD_CELLS_MAX\endcsname{73}
\expandafter\def\csname pv@RD_CELLS_MEAN\endcsname{22.6}
\expandafter\def\csname pv@RD_DIMS_BEST_PHRASE\endcsname{all five}
\expandafter\def\csname pv@RD_EPISODES\endcsname{2{,}100}
\expandafter\def\csname pv@RD_FULL_N\endcsname{Three}
\expandafter\def\csname pv@RD_FULL_TASKS\endcsname{\texttt{stack\_blocks}, \texttt{cover\_blocks}, \texttt{stack\_blocks\_by\_language}}
\expandafter\def\csname pv@RD_INTOK_MEAN_K\endcsname{750}
\expandafter\def\csname pv@RD_LLM_FAILED\endcsname{32.2}
\expandafter\def\csname pv@RD_LLM_MAX\endcsname{76}
\expandafter\def\csname pv@RD_LLM_MEAN\endcsname{25.7}
\expandafter\def\csname pv@RD_LLM_SOLVED\endcsname{19.3}
\expandafter\def\csname pv@RD_LONG_SR\endcsname{48.0}
\expandafter\def\csname pv@RD_MICRO_N\endcsname{2{,}100}
\expandafter\def\csname pv@RD_MICRO_SOLVED\endcsname{1{,}061}
\expandafter\def\csname pv@RD_MICRO_SR\endcsname{50.5}
\expandafter\def\csname pv@RD_OUTTOK_MEAN_K\endcsname{9.0}
\expandafter\def\csname pv@RD_PREC_SR\endcsname{37.3}
\expandafter\def\csname pv@RD_RSI_SCORE\endcsname{36.3}
\expandafter\def\csname pv@RD_RSI_SR\endcsname{31.4}
\expandafter\def\csname pv@RD_SCORE\endcsname{58.2}
\expandafter\def\csname pv@RD_SEED_PHRASE\endcsname{one evaluation seed}
\expandafter\def\csname pv@RD_SR\endcsname{51.6}
\expandafter\def\csname pv@RD_STAR_NOTE\endcsname{}
\expandafter\def\csname pv@RD_TASKS_N\endcsname{42}
\expandafter\def\csname pv@RD_TASK_TIES\endcsname{3}
\expandafter\def\csname pv@RD_TASK_WINS\endcsname{22}
\expandafter\def\csname pv@RD_TOP_NAME\endcsname{VPP2}
\expandafter\def\csname pv@RD_TOP_SCORE\endcsname{39.3}
\expandafter\def\csname pv@RD_TOP_SR\endcsname{32.3}
\expandafter\def\csname pv@RD_USD_EPISODE\endcsname{2.4}
\expandafter\def\csname pv@RD_USD_SEED\endcsname{5{,}100}
\expandafter\def\csname pv@RD_VS_ASTRA_X\endcsname{2.3}
\expandafter\def\csname pv@RD_VS_TOP_SR\endcsname{19.4}
\expandafter\def\csname pv@RD_WALL_MEAN_MIN\endcsname{12.7}
\expandafter\def\csname pv@RD_ZERO_N\endcsname{six}
\expandafter\def\csname pv@RD_ZERO_TASKS\endcsname{\texttt{store\_laptop\_and\_headphones}, \texttt{insert\_key}, \texttt{make\_kong}, \texttt{swap\_blocks}, \texttt{press\_by\_number}, \texttt{store\_tools\_in\_toolbox}}
\expandafter\def\csname pv@S3_COMPOSITE_ALL_COST_RATIO\endcsname{1.4$\times$}
\expandafter\def\csname pv@S3_LIBERO_ALL_COST_RATIO\endcsname{2.5$\times$}
\expandafter\def\csname pv@S3_ROBOCASA_ALL_COST_RATIO\endcsname{1.0$\times$}
\expandafter\def\csname pv@S3_ROBOCASA_ALL_USD_CODE\endcsname{0.96}
\expandafter\def\csname pv@S3_ROBOCASA_ALL_USD_TOOL\endcsname{0.94}
\expandafter\def\csname pv@S3_ROBOTWIN_ALL_COST_RATIO\endcsname{1.6$\times$}
\makeatother


==> generated/values.tex <==
% generated by scripts/paper_numbers.py from data/pyrualean-results.json -- do not edit
\makeatletter
\expandafter\def\csname pv@AB_E4D_BOTH\endcsname{164}
\expandafter\def\csname pv@AB_E4D_CALLS_CODE\endcsname{8.4}
\expandafter\def\csname pv@AB_E4D_CALLS_RPENT\endcsname{21.4}
\expandafter\def\csname pv@AB_E4D_LEAD\endcsname{11.0}
\expandafter\def\csname pv@AB_E4D_N\endcsname{200}
\expandafter\def\csname pv@AB_E4D_PTS\endcsname{+11}
\expandafter\def\csname pv@AB_E4D_PTS_ABS\endcsname{11}
\expandafter\def\csname pv@AB_E4D_RATE_CODE\endcsname{94\%}
\expandafter\def\csname pv@AB_E4D_RATE_RPENT\endcsname{83\%}
\expandafter\def\csname pv@AB_E4D_RATIO_PT\endcsname{4.5$\times$}
\expandafter\def\csname pv@AB_E4D_REQ_CODE\endcsname{8}
\expandafter\def\csname pv@AB_E4D_REQ_RATIO_PT\endcsname{2.5$\times$}
\expandafter\def\csname pv@AB_E4D_REQ_RPENT\endcsname{21}
\expandafter\def\csname pv@AB_E4D_SR_CODE\endcsname{94.0}
\expandafter\def\csname pv@AB_E4D_SR_RPENT\endcsname{83.0}
\expandafter\def\csname pv@AB_E4D_SUCC_CODE\endcsname{188}
\expandafter\def\csname pv@AB_E4D_SUCC_RPENT\endcsname{166}
\expandafter\def\csname pv@AB_NG1_BOTH\endcsname{161}
\expandafter\def\csname pv@AB_NG1_CALLS_CODE\endcsname{9.3}
\expandafter\def\csname pv@AB_NG1_CALLS_RPENT\endcsname{19.0}
\expandafter\def\csname pv@AB_NG1_LEAD\endcsname{4.0}
\expandafter\def\csname pv@AB_NG1_N\endcsname{200}
\expandafter\def\csname pv@AB_NG1_PTS\endcsname{+4}
\expandafter\def\csname pv@AB_NG1_PTS_ABS\endcsname{4}
\expandafter\def\csname pv@AB_NG1_RATE_CODE\endcsname{88\%}
\expandafter\def\csname pv@AB_NG1_RATE_RPENT\endcsname{84\%}
\expandafter\def\csname pv@AB_NG1_RATIO_PT\endcsname{3.1$\times$}
\expandafter\def\csname pv@AB_NG1_REQ_CODE\endcsname{9}
\expandafter\def\csname pv@AB_NG1_REQ_RATIO_PT\endcsname{2.0$\times$}
\expandafter\def\csname pv@AB_NG1_REQ_RPENT\endcsname{19}
\expandafter\def\csname pv@AB_NG1_SR_CODE\endcsname{88.0}
\expandafter\def\csname pv@AB_NG1_SR_RPENT\endcsname{84.0}
\expandafter\def\csname pv@AB_NG1_SUCC_CODE\endcsname{176}
\expandafter\def\csname pv@AB_NG1_SUCC_RPENT\endcsname{168}
\expandafter\def\csname pv@AB_NV1_BOTH\endcsname{126}
\expandafter\def\csname pv@AB_NV1_CALLS_CODE\endcsname{10.9}
\expandafter\def\csname pv@AB_NV1_CALLS_RPENT\endcsname{22.9}
\expandafter\def\csname pv@AB_NV1_LEAD\endcsname{7.5}
\expandafter\def\csname pv@AB_NV1_N\endcsname{200}
\expandafter\def\csname pv@AB_NV1_PTS\endcsname{+8}
\expandafter\def\csname pv@AB_NV1_PTS_ABS\endcsname{8}
\expandafter\def\csname pv@AB_NV1_RATE_CODE\endcsname{80\%}
\expandafter\def\csname pv@AB_NV1_RATE_RPENT\endcsname{73\%}
\expandafter\def\csname pv@AB_NV1_RATIO_PT\endcsname{3.8$\times$}
\expandafter\def\csname pv@AB_NV1_REQ_CODE\endcsname{11}
\expandafter\def\csname pv@AB_NV1_REQ_RATIO_PT\endcsname{2.1$\times$}
\expandafter\def\csname pv@AB_NV1_REQ_RPENT\endcsname{23}
\expandafter\def\csname pv@AB_NV1_SR_CODE\endcsname{80.5}
\expandafter\def\csname pv@AB_NV1_SR_RPENT\endcsname{73.0}
\expandafter\def\csname pv@AB_NV1_SUCC_CODE\endcsname{161}
\expandafter\def\csname pv@AB_NV1_SUCC_RPENT\endcsname{146}
\expandafter\def\csname pv@AB_NVNG1_BOTH\endcsname{130}
\expandafter\def\csname pv@AB_NVNG1_CALLS_CODE\endcsname{9.8}
\expandafter\def\csname pv@AB_NVNG1_CALLS_RPENT\endcsname{20.0}
\expandafter\def\csname pv@AB_NVNG1_LEAD\endcsname{8.0}
\expandafter\def\csname pv@AB_NVNG1_N\endcsname{200}
\expandafter\def\csname pv@AB_NVNG1_PTS\endcsname{+8}
\expandafter\def\csname pv@AB_NVNG1_PTS_ABS\endcsname{8}
\expandafter\def\csname pv@AB_NVNG1_RATE_CODE\endcsname{82\%}
\expandafter\def\csname pv@AB_NVNG1_RATE_RPENT\endcsname{74\%}
\expandafter\def\csname pv@AB_NVNG1_RATIO_PT\endcsname{3.2$\times$}
\expandafter\def\csname pv@AB_NVNG1_REQ_CODE\endcsname{10}
\expandafter\def\csname pv@AB_NVNG1_REQ_RATIO_PT\endcsname{2.0$\times$}
\expandafter\def\csname pv@AB_NVNG1_REQ_RPENT\endcsname{20}
\expandafter\def\csname pv@AB_NVNG1_SR_CODE\endcsname{82.0}
\expandafter\def\csname pv@AB_NVNG1_SR_RPENT\endcsname{74.0}
\expandafter\def\csname pv@AB_NVNG1_SUCC_CODE\endcsname{164}
\expandafter\def\csname pv@AB_NVNG1_SUCC_RPENT\endcsname{148}
\expandafter\def\csname pv@AB_PRICE_RANGE\endcsname{1.1--3.1$\times$}
\expandafter\def\csname pv@AB_RANGE_COMPOSITE\endcsname{2.0--2.3$\times$}
\expandafter\def\csname pv@AB_RANGE_LIBERO\endcsname{3.1--4.5$\times$}
\expandafter\def\csname pv@AB_RANGE_ROBOCASA\endcsname{1.2--1.5$\times$}
\expandafter\def\csname pv@AB_RANGE_ROBOTWIN\endcsname{1.6--3.2$\times$}
\expandafter\def\csname pv@AB_RC1_BOTH\endcsname{69}
\expandafter\def\csname pv@AB_RC1_CALLS_CODE\endcsname{5.6}
\expandafter\def\csname pv@AB_RC1_CALLS_RPENT\endcsname{10.4}
\expandafter\def\csname pv@AB_RC1_LEAD\endcsname{7.8}
\expandafter\def\csname pv@AB_RC1_N\endcsname{90}
\expandafter\def\csname pv@AB_RC1_PTS\endcsname{+8}
\expandafter\def\csname pv@AB_RC1_PTS_ABS\endcsname{8}
\expandafter\def\csname pv@AB_RC1_RATE_CODE\endcsname{87\%}
\expandafter\def\csname pv@AB_RC1_RATE_RPENT\endcsname{79\%}
\expandafter\def\csname pv@AB_RC1_RATIO_PT\endcsname{1.5$\times$}
\expandafter\def\csname pv@AB_RC1_REQ_CODE\endcsname{6}
\expandafter\def\csname pv@AB_RC1_REQ_RATIO_PT\endcsname{1.8$\times$}
\expandafter\def\csname pv@AB_RC1_REQ_RPENT\endcsname{10}
\expandafter\def\csname pv@AB_RC1_SR_CODE\endcsname{86.7}
\expandafter\def\csname pv@AB_RC1_SR_RPENT\endcsname{78.9}
\expandafter\def\csname pv@AB_RC1_SUCC_CODE\endcsname{78}
\expandafter\def\csname pv@AB_RC1_SUCC_RPENT\endcsname{71}
\expandafter\def\csname pv@AB_RCC1_BOTH\endcsname{36}
\expandafter\def\csname pv@AB_RCC1_CALLS_CODE\endcsname{14.9}
\expandafter\def\csname pv@AB_RCC1_CALLS_RPENT\endcsname{28.4}
\expandafter\def\csname pv@AB_RCC1_LEAD\endcsname{5.0}
\expandafter\def\csname pv@AB_RCC1_N\endcsname{160}
\expandafter\def\csname pv@AB_RCC1_PTS\endcsname{+5}
\expandafter\def\csname pv@AB_RCC1_PTS_ABS\endcsname{5}
\expandafter\def\csname pv@AB_RCC1_RATE_CODE\endcsname{39\%}
\expandafter\def\csname pv@AB_RCC1_RATE_RPENT\endcsname{34\%}
\expandafter\def\csname pv@AB_RCC1_RATIO_PT\endcsname{2.0$\times$}
\expandafter\def\csname pv@AB_RCC1_REQ_CODE\endcsname{15}
\expandafter\def\csname pv@AB_RCC1_REQ_RATIO_PT\endcsname{1.9$\times$}
\expandafter\def\csname pv@AB_RCC1_REQ_RPENT\endcsname{28}
\expandafter\def\csname pv@AB_RCC1_SR_CODE\endcsname{39.4}
\expandafter\def\csname pv@AB_RCC1_SR_RPENT\endcsname{34.4}
\expandafter\def\csname pv@AB_RCC1_SUCC_CODE\endcsname{63}
\expandafter\def\csname pv@AB_RCC1_SUCC_RPENT\endcsname{55}
\expandafter\def\csname pv@AB_RCCNV1_BOTH\endcsname{8}
\expandafter\def\csname pv@AB_RCCNV1_CALLS_CODE\endcsname{31.1}
\expandafter\def\csname pv@AB_RCCNV1_CALLS_RPENT\endcsname{58.5}
\expandafter\def\csname pv@AB_RCCNV1_LEAD\endcsname{12.5}
\expandafter\def\csname pv@AB_RCCNV1_N\endcsname{160}
\expandafter\def\csname pv@AB_RCCNV1_PTS\endcsname{+12}
\expandafter\def\csname pv@AB_RCCNV1_PTS_ABS\endcsname{12}
\expandafter\def\csname pv@AB_RCCNV1_RATE_CODE\endcsname{20\%}
\expandafter\def\csname pv@AB_RCCNV1_RATE_RPENT\endcsname{8\%}
\expandafter\def\csname pv@AB_RCCNV1_RATIO_PT\endcsname{2.3$\times$}
\expandafter\def\csname pv@AB_RCCNV1_REQ_CODE\endcsname{31}
\expandafter\def\csname pv@AB_RCCNV1_REQ_RATIO_PT\endcsname{1.9$\times$}
\expandafter\def\csname pv@AB_RCCNV1_REQ_RPENT\endcsname{58}
\expandafter\def\csname pv@AB_RCCNV1_SR_CODE\endcsname{20.0}
\expandafter\def\csname pv@AB_RCCNV1_SR_RPENT\endcsname{7.5}
\expandafter\def\csname pv@AB_RCCNV1_SUCC_CODE\endcsname{32}
\expandafter\def\csname pv@AB_RCCNV1_SUCC_RPENT\endcsname{12}
\expandafter\def\csname pv@AB_RCNV1_BOTH\endcsname{35}
\expandafter\def\csname pv@AB_RCNV1_CALLS_CODE\endcsname{18.7}
\expandafter\def\csname pv@AB_RCNV1_CALLS_RPENT\endcsname{26.5}
\expandafter\def\csname pv@AB_RCNV1_LEAD\endcsname{20.0}
\expandafter\def\csname pv@AB_RCNV1_N\endcsname{90}
\expandafter\def\csname pv@AB_RCNV1_PTS\endcsname{+20}
\expandafter\def\csname pv@AB_RCNV1_PTS_ABS\endcsname{20}
\expandafter\def\csname pv@AB_RCNV1_RATE_CODE\endcsname{66\%}
\expandafter\def\csname pv@AB_RCNV1_RATE_RPENT\endcsname{46\%}
\expandafter\def\csname pv@AB_RCNV1_RATIO_PT\endcsname{1.2$\times$}
\expandafter\def\csname pv@AB_RCNV1_REQ_CODE\endcsname{19}
\expandafter\def\csname pv@AB_RCNV1_REQ_RATIO_PT\endcsname{1.4$\times$}
\expandafter\def\csname pv@AB_RCNV1_REQ_RPENT\endcsname{27}
\expandafter\def\csname pv@AB_RCNV1_SR_CODE\endcsname{65.6}
\expandafter\def\csname pv@AB_RCNV1_SR_RPENT\endcsname{45.6}
\expandafter\def\csname pv@AB_RCNV1_SUCC_CODE\endcsname{59}
\expandafter\def\csname pv@AB_RCNV1_SUCC_RPENT\endcsname{41}
\expandafter\def\csname pv@AB_RT1_BOTH\endcsname{137}
\expandafter\def\csname pv@AB_RT1_CALLS_CODE\endcsname{8.9}
\expandafter\def\csname pv@AB_RT1_CALLS_RPENT\endcsname{12.2}
\expandafter\def\csname pv@AB_RT1_LEAD\endcsname{9.2}
\expandafter\def\csname pv@AB_RT1_N\endcsname{250}
\expandafter\def\csname pv@AB_RT1_PTS\endcsname{+9}
\expandafter\def\csname pv@AB_RT1_PTS_ABS\endcsname{9}
\expandafter\def\csname pv@AB_RT1_RATE_CODE\endcsname{69\%}
\expandafter\def\csname pv@AB_RT1_RATE_RPENT\endcsname{60\%}
\expandafter\def\csname pv@AB_RT1_RATIO_PT\endcsname{1.7$\times$}
\expandafter\def\csname pv@AB_RT1_REQ_CODE\endcsname{9}
\expandafter\def\csname pv@AB_RT1_REQ_RATIO_PT\endcsname{1.4$\times$}
\expandafter\def\csname pv@AB_RT1_REQ_RPENT\endcsname{12}
\expandafter\def\csname pv@AB_RT1_SR_CODE\endcsname{69.2}
\expandafter\def\csname pv@AB_RT1_SR_RPENT\endcsname{60.0}
\expandafter\def\csname pv@AB_RT1_SUCC_CODE\endcsname{173}
\expandafter\def\csname pv@AB_RT1_SUCC_RPENT\endcsname{150}
\expandafter\def\csname pv@AB_RTNG1_BOTH\endcsname{136}
\expandafter\def\csname pv@AB_RTNG1_CALLS_CODE\endcsname{9.1}
\expandafter\def\csname pv@AB_RTNG1_CALLS_RPENT\endcsname{11.6}
\expandafter\def\csname pv@AB_RTNG1_LEAD\endcsname{2.8}
\expandafter\def\csname pv@AB_RTNG1_N\endcsname{250}
\expandafter\def\csname pv@AB_RTNG1_PTS\endcsname{+3}
\expandafter\def\csname pv@AB_RTNG1_PTS_ABS\endcsname{3}
\expandafter\def\csname pv@AB_RTNG1_RATE_CODE\endcsname{67\%}
\expandafter\def\csname pv@AB_RTNG1_RATE_RPENT\endcsname{64\%}
\expandafter\def\csname pv@AB_RTNG1_RATIO_PT\endcsname{1.6$\times$}
\expandafter\def\csname pv@AB_RTNG1_REQ_CODE\endcsname{9}
\expandafter\def\csname pv@AB_RTNG1_REQ_RATIO_PT\endcsname{1.3$\times$}
\expandafter\def\csname pv@AB_RTNG1_REQ_RPENT\endcsname{12}
\expandafter\def\csname pv@AB_RTNG1_SR_CODE\endcsname{66.8}
\expandafter\def\csname pv@AB_RTNG1_SR_RPENT\endcsname{64.0}
\expandafter\def\csname pv@AB_RTNG1_SUCC_CODE\endcsname{167}
\expandafter\def\csname pv@AB_RTNG1_SUCC_RPENT\endcsname{160}
\expandafter\def\csname pv@AB_RTNV1_BOTH\endcsname{94}
\expandafter\def\csname pv@AB_RTNV1_CALLS_CODE\endcsname{11.5}
\expandafter\def\csname pv@AB_RTNV1_CALLS_RPENT\endcsname{23.1}
\expandafter\def\csname pv@AB_RTNV1_LEAD\endcsname{26.0}
\expandafter\def\csname pv@AB_RTNV1_N\endcsname{250}
\expandafter\def\csname pv@AB_RTNV1_PTS\endcsname{+26}
\expandafter\def\csname pv@AB_RTNV1_PTS_ABS\endcsname{26}
\expandafter\def\csname pv@AB_RTNV1_RATE_CODE\endcsname{69\%}
\expandafter\def\csname pv@AB_RTNV1_RATE_RPENT\endcsname{43\%}
\expandafter\def\csname pv@AB_RTNV1_RATIO_PT\endcsname{3.2$\times$}
\expandafter\def\csname pv@AB_RTNV1_REQ_CODE\endcsname{11}
\expandafter\def\csname pv@AB_RTNV1_REQ_RATIO_PT\endcsname{2.0$\times$}
\expandafter\def\csname pv@AB_RTNV1_REQ_RPENT\endcsname{23}
\expandafter\def\csname pv@AB_RTNV1_SR_CODE\endcsname{68.8}
\expandafter\def\csname pv@AB_RTNV1_SR_RPENT\endcsname{42.8}
\expandafter\def\csname pv@AB_RTNV1_SUCC_CODE\endcsname{172}
\expandafter\def\csname pv@AB_RTNV1_SUCC_RPENT\endcsname{107}
\expandafter\def\csname pv@AB_RTNVNG1_BOTH\endcsname{118}
\expandafter\def\csname pv@AB_RTNVNG1_CALLS_CODE\endcsname{12.0}
\expandafter\def\csname pv@AB_RTNVNG1_CALLS_RPENT\endcsname{16.9}
\expandafter\def\csname pv@AB_RTNVNG1_LEAD\endcsname{6.0}
\expandafter\def\csname pv@AB_RTNVNG1_N\endcsname{250}
\expandafter\def\csname pv@AB_RTNVNG1_PTS\endcsname{+6}
\expandafter\def\csname pv@AB_RTNVNG1_PTS_ABS\endcsname{6}
\expandafter\def\csname pv@AB_RTNVNG1_RATE_CODE\endcsname{66\%}
\expandafter\def\csname pv@AB_RTNVNG1_RATE_RPENT\endcsname{60\%}
\expandafter\def\csname pv@AB_RTNVNG1_RATIO_PT\endcsname{1.9$\times$}
\expandafter\def\csname pv@AB_RTNVNG1_REQ_CODE\endcsname{12}
\expandafter\def\csname pv@AB_RTNVNG1_REQ_RATIO_PT\endcsname{1.4$\times$}
\expandafter\def\csname pv@AB_RTNVNG1_REQ_RPENT\endcsname{17}
\expandafter\def\csname pv@AB_RTNVNG1_SR_CODE\endcsname{66.4}
\expandafter\def\csname pv@AB_RTNVNG1_SR_RPENT\endcsname{60.4}
\expandafter\def\csname pv@AB_RTNVNG1_SUCC_CODE\endcsname{166}
\expandafter\def\csname pv@AB_RTNVNG1_SUCC_RPENT\endcsname{151}
\expandafter\def\csname pv@AB_SCOPE\endcsname{all 200 of LIBERO-PRO's task instances, all 250 of RoboTwin~2.0's, all 90 of RoboCasa365's atomic ones and all 160 of its composite ones}
\expandafter\def\csname pv@AB_SETTINGS\endcsname{8}
\expandafter\def\csname pv@ACTING_PAIRS\endcsname{45}
\expandafter\def\csname pv@ACT_PER_CELL\endcsname{2.1}
\expandafter\def\csname pv@ACT_PER_TOOLCALL\endcsname{0.65}
\expandafter\def\csname pv@BOTH_SOLVED_N\endcsname{406}
\expandafter\def\csname pv@CAP_TIMES\endcsname{1.2 to 3.6 times}
\expandafter\def\csname pv@CARRY_SHARE\endcsname{19\%}
\expandafter\def\csname pv@CELLS_FAILED\endcsname{32.6}
\expandafter\def\csname pv@CELLS_SOLVED\endcsname{9.3}
\expandafter\def\csname pv@CODE_CELLS_N\endcsname{11,145}
\expandafter\def\csname pv@CODE_EPISODES_N\endcsname{700}
\expandafter\def\csname pv@CODE_ONLY_CAP\endcsname{52}
\expandafter\def\csname pv@CODE_ONLY_ENDED\endcsname{44}
\expandafter\def\csname pv@CODE_ONLY_N\endcsname{96}
\expandafter\def\csname pv@COMPOSITE_ALL_RATIO_1\endcsname{1.6$\times$}
\expandafter\def\csname pv@COMPOSITE_ALL_RATIO_PT\endcsname{1.57$\times$}
\expandafter\def\csname pv@COMPOSITE_AT05M_CODE\endcsname{23\%}
\expandafter\def\csname pv@COMPOSITE_AT05M_RPENT\endcsname{18\%}
\expandafter\def\csname pv@COMPOSITE_AT10M_CODE\endcsname{29\%}
\expandafter\def\csname pv@COMPOSITE_AT10M_RPENT\endcsname{23\%}
\expandafter\def\csname pv@COMPOSITE_AT30M_CODE\endcsname{38\%}
\expandafter\def\csname pv@COMPOSITE_AT30M_RPENT\endcsname{31\%}
\expandafter\def\csname pv@COMPOSITE_BOTH\endcsname{36}
\expandafter\def\csname pv@COMPOSITE_BUDGET\endcsname{100}
\expandafter\def\csname pv@COMPOSITE_CAP_RATE_CODE\endcsname{0.6\%}
\expandafter\def\csname pv@COMPOSITE_CAP_RATE_RPENT\endcsname{4.4\%}
\expandafter\def\csname pv@COMPOSITE_CAP_SHARE_CODE\endcsname{1\%}
\expandafter\def\csname pv@COMPOSITE_CAP_SHARE_RPENT\endcsname{7\%}
\expandafter\def\csname pv@COMPOSITE_CHEAPER\endcsname{64\%}
\expandafter\def\csname pv@COMPOSITE_FIRST_CODE\endcsname{24k}
\expandafter\def\csname pv@COMPOSITE_FIRST_RPENT\endcsname{17k}
\expandafter\def\csname pv@COMPOSITE_GAVEUP_DEC_CODE\endcsname{34}
\expandafter\def\csname pv@COMPOSITE_GAVEUP_DEC_RPENT\endcsname{49}
\expandafter\def\csname pv@COMPOSITE_MEAN_TOK_CODE\endcsname{603k}
\expandafter\def\csname pv@COMPOSITE_MEAN_TOK_RPENT\endcsname{1.22M}
\expandafter\def\csname pv@COMPOSITE_MEDIAN_PT\endcsname{1.66$\times$}
\expandafter\def\csname pv@COMPOSITE_N\endcsname{160}
\expandafter\def\csname pv@COMPOSITE_OUT_CODE_X\endcsname{0.8$\times$}
\expandafter\def\csname pv@COMPOSITE_OUT_SHARE_CODE\endcsname{17\%}
\expandafter\def\csname pv@COMPOSITE_OUT_SHARE_RPENT\endcsname{14\%}
\expandafter\def\csname pv@COMPOSITE_PER_CALL_CODE\endcsname{40k}
\expandafter\def\csname pv@COMPOSITE_PER_CALL_RPENT\endcsname{43k}
\expandafter\def\csname pv@COMPOSITE_PRICE_PT\endcsname{1.6$\times$}
\expandafter\def\csname pv@COMPOSITE_PTS\endcsname{+5.0}
\expandafter\def\csname pv@COMPOSITE_PTS_ABS\endcsname{5.0}
\expandafter\def\csname pv@COMPOSITE_RATE_CODE\endcsname{39.4\%}
\expandafter\def\csname pv@COMPOSITE_RATE_RPENT\endcsname{34.4\%}
\expandafter\def\csname pv@COMPOSITE_RATIO_PT\endcsname{2.0$\times$}
\expandafter\def\csname pv@COMPOSITE_RATIO_X2\endcsname{2.03$\times$}
\expandafter\def\csname pv@COMPOSITE_REACH_CODE\endcsname{1.98M}
\expandafter\def\csname pv@COMPOSITE_REACH_LEVEL\endcsname{34.4\%}
\expandafter\def\csname pv@COMPOSITE_REACH_REQ_CODE\endcsname{42}
\expandafter\def\csname pv@COMPOSITE_REACH_REQ_RPENT\endcsname{90}
\expandafter\def\csname pv@COMPOSITE_REACH_REQ_X\endcsname{2.1$\times$}
\expandafter\def\csname pv@COMPOSITE_REACH_RPENT\endcsname{5.71M}
\expandafter\def\csname pv@COMPOSITE_REACH_X\endcsname{2.9$\times$}
\expandafter\def\csname pv@COMPOSITE_REQ1_CODE\endcsname{14.9}
\expandafter\def\csname pv@COMPOSITE_REQ1_RPENT\endcsname{28.4}
\expandafter\def\csname pv@COMPOSITE_REQ_CODE\endcsname{15}
\expandafter\def\csname pv@COMPOSITE_REQ_RATIO_PT\endcsname{1.9$\times$}
\expandafter\def\csname pv@COMPOSITE_REQ_RATIO_X2\endcsname{1.90$\times$}
\expandafter\def\csname pv@COMPOSITE_REQ_RPENT\endcsname{28}
\expandafter\def\csname pv@COMPOSITE_STEPS_CODE_X\endcsname{1.2$\times$}
\expandafter\def\csname pv@COMPOSITE_SUCC_CODE\endcsname{63}
\expandafter\def\csname pv@COMPOSITE_SUCC_RPENT\endcsname{55}
\expandafter\def\csname pv@COMPOSITE_TASKS\endcsname{32}
\expandafter\def\csname pv@COMPOSITE_TPR_RATIO_PT\endcsname{1.1$\times$}
\expandafter\def\csname pv@COMPOSITE_TPR_RATIO_X2\endcsname{1.06$\times$}
\expandafter\def\csname pv@COMPOSITE_TTS_CODE\endcsname{164k}
\expandafter\def\csname pv@COMPOSITE_TTS_DEC_CODE\endcsname{6}
\expandafter\def\csname pv@COMPOSITE_TTS_DEC_RPENT\endcsname{14}
\expandafter\def\csname pv@COMPOSITE_TTS_RPENT\endcsname{312k}
\expandafter\def\csname pv@COMPOSITE_USD_CODE\endcsname{\$1.25}
\expandafter\def\csname pv@COMPOSITE_USD_RPENT\endcsname{\$2.01}
\expandafter\def\csname pv@CONDLOOK_SHARE\endcsname{20\%}
\expandafter\def\csname pv@DEF_SHARE\endcsname{2\%}
\expandafter\def\csname pv@DEMO_CALLS_CODE\endcsname{8}
\expandafter\def\csname pv@DEMO_CALLS_RPENT\endcsname{20}
\expandafter\def\csname pv@DEMO_IMAGES_CODE\endcsname{5}
\expandafter\def\csname pv@DEMO_IMAGES_RPENT\endcsname{33}
\expandafter\def\csname pv@DEMO_SOLVED_CODE\endcsname{6}
\expandafter\def\csname pv@DEMO_SOLVED_RPENT\endcsname{17}
\expandafter\def\csname pv@DEMO_TASK\endcsname{Pick the akita black bowl on the stove and place it on the plate}
\expandafter\def\csname pv@DEMO_TOK_CODE\endcsname{220k}
\expandafter\def\csname pv@DEMO_TOK_RPENT\endcsname{1.04M}
\expandafter\def\csname pv@DEMO_TOK_SOLVED_CODE\endcsname{156k}
\expandafter\def\csname pv@DEMO_TOK_SOLVED_RPENT\endcsname{816k}
\expandafter\def\csname pv@EXAMPLE_GUARDED_CELL\endcsname{2}
\expandafter\def\csname pv@EXAMPLE_GUARDED_EPISODE\endcsname{LIBERO-PRO, spatial swap, task 0, seed 0}
\expandafter\def\csname pv@EXAMPLE_PERCEPTION_CELL\endcsname{5}
\expandafter\def\csname pv@EXAMPLE_PERCEPTION_EPISODE\endcsname{RoboTwin 2.0 without the VLA policy, handover block, seed 100003}
\expandafter\def\csname pv@EXAMPLE_SKILL_CELL\endcsname{7}
\expandafter\def\csname pv@EXAMPLE_SKILL_EPISODE\endcsname{RoboTwin 2.0, place object stand, seed 100002}
\expandafter\def\csname pv@FIT_GAP\endcsname{4}
\expandafter\def\csname pv@GUARDED_LIBERO\endcsname{45\%}
\expandafter\def\csname pv@GUARDED_SHARE\endcsname{19\%}
\expandafter\def\csname pv@HELPER_SHARE\endcsname{7\%}
\expandafter\def\csname pv@LIBERO_ALL_RATIO_1\endcsname{3.1$\times$}
\expandafter\def\csname pv@LIBERO_ALL_RATIO_PT\endcsname{3.08$\times$}
\expandafter\def\csname pv@LIBERO_AT05M_CODE\endcsname{81\%}
\expandafter\def\csname pv@LIBERO_AT05M_RPENT\endcsname{6\%}
\expandafter\def\csname pv@LIBERO_AT10M_CODE\endcsname{88\%}
\expandafter\def\csname pv@LIBERO_AT10M_RPENT\endcsname{55\%}
\expandafter\def\csname pv@LIBERO_AT30M_CODE\endcsname{94\%}
\expandafter\def\csname pv@LIBERO_AT30M_RPENT\endcsname{82\%}
\expandafter\def\csname pv@LIBERO_BOTH\endcsname{164}
\expandafter\def\csname pv@LIBERO_BUDGET\endcsname{40}
\expandafter\def\csname pv@LIBERO_CAP_RATE_CODE\endcsname{3.5\%}
\expandafter\def\csname pv@LIBERO_CAP_RATE_RPENT\endcsname{12.5\%}
\expandafter\def\csname pv@LIBERO_CAP_SHARE_CODE\endcsname{58\%}
\expandafter\def\csname pv@LIBERO_CAP_SHARE_RPENT\endcsname{74\%}
\expandafter\def\csname pv@LIBERO_CHEAPER\endcsname{100\%}
\expandafter\def\csname pv@LIBERO_FIRST_CODE\endcsname{22k}
\expandafter\def\csname pv@LIBERO_FIRST_RPENT\endcsname{20k}
\expandafter\def\csname pv@LIBERO_GAVEUP_DEC_CODE\endcsname{27}
\expandafter\def\csname pv@LIBERO_GAVEUP_DEC_RPENT\endcsname{35}
\expandafter\def\csname pv@LIBERO_MEAN_TOK_CODE\endcsname{273k}
\expandafter\def\csname pv@LIBERO_MEAN_TOK_RPENT\endcsname{1.23M}
\expandafter\def\csname pv@LIBERO_MEDIAN_PT\endcsname{4.83$\times$}
\expandafter\def\csname pv@LIBERO_N\endcsname{200}
\expandafter\def\csname pv@LIBERO_OUT_CODE_X\endcsname{0.3$\times$}
\expandafter\def\csname pv@LIBERO_OUT_SHARE_CODE\endcsname{13\%}
\expandafter\def\csname pv@LIBERO_OUT_SHARE_RPENT\endcsname{13\%}
\expandafter\def\csname pv@LIBERO_PER_CALL_CODE\endcsname{33k}
\expandafter\def\csname pv@LIBERO_PER_CALL_RPENT\endcsname{57k}
\expandafter\def\csname pv@LIBERO_PRICE_PT\endcsname{3.1$\times$}
\expandafter\def\csname pv@LIBERO_PTS\endcsname{+11.0}
\expandafter\def\csname pv@LIBERO_PTS_ABS\endcsname{11.0}
\expandafter\def\csname pv@LIBERO_RATE_CODE\endcsname{94.0\%}
\expandafter\def\csname pv@LIBERO_RATE_RPENT\endcsname{83.0\%}
\expandafter\def\csname pv@LIBERO_RATIO_PT\endcsname{4.5$\times$}
\expandafter\def\csname pv@LIBERO_RATIO_X2\endcsname{4.48$\times$}
\expandafter\def\csname pv@LIBERO_REACH_CODE\endcsname{564k}
\expandafter\def\csname pv@LIBERO_REACH_LEVEL\endcsname{83.0\%}
\expandafter\def\csname pv@LIBERO_REACH_REQ_CODE\endcsname{14}
\expandafter\def\csname pv@LIBERO_REACH_REQ_RPENT\endcsname{39}
\expandafter\def\csname pv@LIBERO_REACH_REQ_X\endcsname{2.8$\times$}
\expandafter\def\csname pv@LIBERO_REACH_RPENT\endcsname{3.18M}
\expandafter\def\csname pv@LIBERO_REACH_X\endcsname{5.6$\times$}
\expandafter\def\csname pv@LIBERO_REQ1_CODE\endcsname{8.4}
\expandafter\def\csname pv@LIBERO_REQ1_RPENT\endcsname{21.4}
\expandafter\def\csname pv@LIBERO_REQ_CODE\endcsname{8}
\expandafter\def\csname pv@LIBERO_REQ_RATIO_PT\endcsname{2.5$\times$}
\expandafter\def\csname pv@LIBERO_REQ_RATIO_X2\endcsname{2.55$\times$}
\expandafter\def\csname pv@LIBERO_REQ_RPENT\endcsname{21}
\expandafter\def\csname pv@LIBERO_STEPS_CODE_X\endcsname{0.9$\times$}
\expandafter\def\csname pv@LIBERO_SUCC_CODE\endcsname{188}
\expandafter\def\csname pv@LIBERO_SUCC_RPENT\endcsname{166}
\expandafter\def\csname pv@LIBERO_TASKS\endcsname{40}
\expandafter\def\csname pv@LIBERO_TPR_RATIO_PT\endcsname{1.8$\times$}
\expandafter\def\csname pv@LIBERO_TPR_RATIO_X2\endcsname{1.76$\times$}
\expandafter\def\csname pv@LIBERO_TTS_CODE\endcsname{133k}
\expandafter\def\csname pv@LIBERO_TTS_DEC_CODE\endcsname{5}
\expandafter\def\csname pv@LIBERO_TTS_DEC_RPENT\endcsname{16}
\expandafter\def\csname pv@LIBERO_TTS_RPENT\endcsname{767k}
\expandafter\def\csname pv@LIBERO_USD_CODE\endcsname{\$0.79}
\expandafter\def\csname pv@LIBERO_USD_RPENT\endcsname{\$2.49}
\expandafter\def\csname pv@MULTI_BP\endcsname{1,441}
\expandafter\def\csname pv@MULTI_CALLS\endcsname{1,907}
\expandafter\def\csname pv@MULTI_FILE\endcsname{292}
\expandafter\def\csname pv@NUMPY_SHARE\endcsname{30\%}
\expandafter\def\csname pv@OD_CALLS_AUTO\endcsname{19.9}
\expandafter\def\csname pv@OD_CALLS_CODE\endcsname{7.4}
\expandafter\def\csname pv@OD_CALLS_OD\endcsname{22.8}
\expandafter\def\csname pv@OD_COMMON\endcsname{131}
\expandafter\def\csname pv@OD_N\endcsname{200}
\expandafter\def\csname pv@OD_SR_AUTO\endcsname{83.0}
\expandafter\def\csname pv@OD_SR_CODE\endcsname{94.0}
\expandafter\def\csname pv@OD_SR_OD\endcsname{68.5}
\expandafter\def\csname pv@OD_TOK_AUTO\endcsname{1.07M}
\expandafter\def\csname pv@OD_TOK_CODE\endcsname{222k}
\expandafter\def\csname pv@OD_TOK_OD\endcsname{1.07M}
\expandafter\def\csname pv@OD_TOK_X\endcsname{4.8$\times$}
\expandafter\def\csname pv@OUT_SHARE_MAX\endcsname{17\%}
\expandafter\def\csname pv@POOLED_CALLS_PHRASE\endcsname{half as many}
\expandafter\def\csname pv@POOLED_N\endcsname{700}
\expandafter\def\csname pv@POOLED_PRICEF\endcsname{2.2$\times$}
\expandafter\def\csname pv@POOLED_PTS\endcsname{+8.6}
\expandafter\def\csname pv@POOLED_REQF\endcsname{2.0$\times$}
\expandafter\def\csname pv@POOLED_SR_CODE\endcsname{71.7\%}
\expandafter\def\csname pv@POOLED_SR_REL\endcsname{14\%}
\expandafter\def\csname pv@POOLED_SR_RPENT\endcsname{63.1\%}
\expandafter\def\csname pv@POOLED_TOKENS_FEWER\endcsname{65\%}
\expandafter\def\csname pv@POOLED_TOKEN_FACTOR\endcsname{2.9$\times$}
\expandafter\def\csname pv@PRICEF_RANGE\endcsname{1.2--3.1$\times$}
\expandafter\def\csname pv@PTS_RANGE\endcsname{+5.0 to +11.0}
\expandafter\def\csname pv@REACH_REQ_RANGE\endcsname{2.0--2.8$\times$}
\expandafter\def\csname pv@RETRY_CELL\endcsname{1}
\expandafter\def\csname pv@RETRY_EPISODE\endcsname{RoboCasa365 atomic, CloseToasterOvenDoor, seed 1}
\expandafter\def\csname pv@RETRY_ROBOCASA\endcsname{18\%}
\expandafter\def\csname pv@RETRY_SHARE\endcsname{8\%}
\expandafter\def\csname pv@ROBOCASA_ALL_RATIO_1\endcsname{1.1$\times$}
\expandafter\def\csname pv@ROBOCASA_ALL_RATIO_PT\endcsname{1.11$\times$}
\expandafter\def\csname pv@ROBOCASA_AT05M_CODE\endcsname{73\%}
\expandafter\def\csname pv@ROBOCASA_AT05M_RPENT\endcsname{69\%}
\expandafter\def\csname pv@ROBOCASA_AT10M_CODE\endcsname{82\%}
\expandafter\def\csname pv@ROBOCASA_AT10M_RPENT\endcsname{74\%}
\expandafter\def\csname pv@ROBOCASA_AT30M_CODE\endcsname{87\%}
\expandafter\def\csname pv@ROBOCASA_AT30M_RPENT\endcsname{79\%}
\expandafter\def\csname pv@ROBOCASA_BOTH\endcsname{69}
\expandafter\def\csname pv@ROBOCASA_BUDGET\endcsname{40}
\expandafter\def\csname pv@ROBOCASA_CAP_RATE_CODE\endcsname{6.7\%}
\expandafter\def\csname pv@ROBOCASA_CAP_RATE_RPENT\endcsname{11.1\%}
\expandafter\def\csname pv@ROBOCASA_CAP_SHARE_CODE\endcsname{50\%}
\expandafter\def\csname pv@ROBOCASA_CAP_SHARE_RPENT\endcsname{53\%}
\expandafter\def\csname pv@ROBOCASA_CHEAPER\endcsname{88\%}
\expandafter\def\csname pv@ROBOCASA_FIRST_CODE\endcsname{24k}
\expandafter\def\csname pv@ROBOCASA_FIRST_RPENT\endcsname{17k}
\expandafter\def\csname pv@ROBOCASA_GAVEUP_DEC_CODE\endcsname{29}
\expandafter\def\csname pv@ROBOCASA_GAVEUP_DEC_RPENT\endcsname{30}
\expandafter\def\csname pv@ROBOCASA_MEAN_TOK_CODE\endcsname{171k}
\expandafter\def\csname pv@ROBOCASA_MEAN_TOK_RPENT\endcsname{261k}
\expandafter\def\csname pv@ROBOCASA_MEDIAN_PT\endcsname{1.49$\times$}
\expandafter\def\csname pv@ROBOCASA_N\endcsname{90}
\expandafter\def\csname pv@ROBOCASA_OUT_CODE_X\endcsname{0.8$\times$}
\expandafter\def\csname pv@ROBOCASA_OUT_SHARE_CODE\endcsname{10\%}
\expandafter\def\csname pv@ROBOCASA_OUT_SHARE_RPENT\endcsname{11\%}
\expandafter\def\csname pv@ROBOCASA_PER_CALL_CODE\endcsname{30k}
\expandafter\def\csname pv@ROBOCASA_PER_CALL_RPENT\endcsname{25k}
\expandafter\def\csname pv@ROBOCASA_PRICE_PT\endcsname{1.2$\times$}
\expandafter\def\csname pv@ROBOCASA_PTS\endcsname{+7.8}
\expandafter\def\csname pv@ROBOCASA_PTS_ABS\endcsname{7.8}
\expandafter\def\csname pv@ROBOCASA_RATE_CODE\endcsname{86.7\%}
\expandafter\def\csname pv@ROBOCASA_RATE_RPENT\endcsname{78.9\%}
\expandafter\def\csname pv@ROBOCASA_RATIO_PT\endcsname{1.5$\times$}
\expandafter\def\csname pv@ROBOCASA_RATIO_X2\endcsname{1.53$\times$}
\expandafter\def\csname pv@ROBOCASA_REACH_CODE\endcsname{619k}
\expandafter\def\csname pv@ROBOCASA_REACH_LEVEL\endcsname{78.9\%}
\expandafter\def\csname pv@ROBOCASA_REACH_REQ_CODE\endcsname{18}
\expandafter\def\csname pv@ROBOCASA_REACH_REQ_RPENT\endcsname{38}
\expandafter\def\csname pv@ROBOCASA_REACH_REQ_X\endcsname{2.1$\times$}
\expandafter\def\csname pv@ROBOCASA_REACH_RPENT\endcsname{1.32M}
\expandafter\def\csname pv@ROBOCASA_REACH_X\endcsname{2.1$\times$}
\expandafter\def\csname pv@ROBOCASA_REQ1_CODE\endcsname{5.6}
\expandafter\def\csname pv@ROBOCASA_REQ1_RPENT\endcsname{10.4}
\expandafter\def\csname pv@ROBOCASA_REQ_CODE\endcsname{6}
\expandafter\def\csname pv@ROBOCASA_REQ_RATIO_PT\endcsname{1.8$\times$}
\expandafter\def\csname pv@ROBOCASA_REQ_RATIO_X2\endcsname{1.84$\times$}
\expandafter\def\csname pv@ROBOCASA_REQ_RPENT\endcsname{10}
\expandafter\def\csname pv@ROBOCASA_STEPS_CODE_X\endcsname{1.1$\times$}
\expandafter\def\csname pv@ROBOCASA_SUCC_CODE\endcsname{78}
\expandafter\def\csname pv@ROBOCASA_SUCC_RPENT\endcsname{71}
\expandafter\def\csname pv@ROBOCASA_TASKS\endcsname{18}
\expandafter\def\csname pv@ROBOCASA_TPR_RATIO_PT\endcsname{0.8$\times$}
\expandafter\def\csname pv@ROBOCASA_TPR_RATIO_X2\endcsname{0.83$\times$}
\expandafter\def\csname pv@ROBOCASA_TTS_CODE\endcsname{24k}
\expandafter\def\csname pv@ROBOCASA_TTS_DEC_CODE\endcsname{1}
\expandafter\def\csname pv@ROBOCASA_TTS_DEC_RPENT\endcsname{4}
\expandafter\def\csname pv@ROBOCASA_TTS_RPENT\endcsname{72k}
\expandafter\def\csname pv@ROBOCASA_USD_CODE\endcsname{\$0.54}
\expandafter\def\csname pv@ROBOCASA_USD_RPENT\endcsname{\$0.62}
\expandafter\def\csname pv@ROBOTWIN_ALL_RATIO_1\endcsname{1.8$\times$}
\expandafter\def\csname pv@ROBOTWIN_ALL_RATIO_PT\endcsname{1.78$\times$}
\expandafter\def\csname pv@ROBOTWIN_AT05M_CODE\endcsname{55\%}
\expandafter\def\csname pv@ROBOTWIN_AT05M_RPENT\endcsname{48\%}
\expandafter\def\csname pv@ROBOTWIN_AT10M_CODE\endcsname{67\%}
\expandafter\def\csname pv@ROBOTWIN_AT10M_RPENT\endcsname{54\%}
\expandafter\def\csname pv@ROBOTWIN_AT30M_CODE\endcsname{69\%}
\expandafter\def\csname pv@ROBOTWIN_AT30M_RPENT\endcsname{60\%}
\expandafter\def\csname pv@ROBOTWIN_BOTH\endcsname{137}
\expandafter\def\csname pv@ROBOTWIN_BUDGET\endcsname{40}
\expandafter\def\csname pv@ROBOTWIN_CAP_RATE_CODE\endcsname{15.2\%}
\expandafter\def\csname pv@ROBOTWIN_CAP_RATE_RPENT\endcsname{18.4\%}
\expandafter\def\csname pv@ROBOTWIN_CAP_SHARE_CODE\endcsname{49\%}
\expandafter\def\csname pv@ROBOTWIN_CAP_SHARE_RPENT\endcsname{46\%}
\expandafter\def\csname pv@ROBOTWIN_CHEAPER\endcsname{85\%}
\expandafter\def\csname pv@ROBOTWIN_FIRST_CODE\endcsname{21k}
\expandafter\def\csname pv@ROBOTWIN_FIRST_RPENT\endcsname{15k}
\expandafter\def\csname pv@ROBOTWIN_GAVEUP_DEC_CODE\endcsname{21}
\expandafter\def\csname pv@ROBOTWIN_GAVEUP_DEC_RPENT\endcsname{24}
\expandafter\def\csname pv@ROBOTWIN_MEAN_TOK_CODE\endcsname{245k}
\expandafter\def\csname pv@ROBOTWIN_MEAN_TOK_RPENT\endcsname{415k}
\expandafter\def\csname pv@ROBOTWIN_MEDIAN_PT\endcsname{1.58$\times$}
\expandafter\def\csname pv@ROBOTWIN_N\endcsname{250}
\expandafter\def\csname pv@ROBOTWIN_OUT_CODE_X\endcsname{1.2$\times$}
\expandafter\def\csname pv@ROBOTWIN_OUT_SHARE_CODE\endcsname{14\%}
\expandafter\def\csname pv@ROBOTWIN_OUT_SHARE_RPENT\endcsname{8\%}
\expandafter\def\csname pv@ROBOTWIN_PER_CALL_CODE\endcsname{28k}
\expandafter\def\csname pv@ROBOTWIN_PER_CALL_RPENT\endcsname{34k}
\expandafter\def\csname pv@ROBOTWIN_PRICE_PT\endcsname{1.5$\times$}
\expandafter\def\csname pv@ROBOTWIN_PTS\endcsname{+9.2}
\expandafter\def\csname pv@ROBOTWIN_PTS_ABS\endcsname{9.2}
\expandafter\def\csname pv@ROBOTWIN_RATE_CODE\endcsname{69.2\%}
\expandafter\def\csname pv@ROBOTWIN_RATE_RPENT\endcsname{60.0\%}
\expandafter\def\csname pv@ROBOTWIN_RATIO_PT\endcsname{1.7$\times$}
\expandafter\def\csname pv@ROBOTWIN_RATIO_X2\endcsname{1.69$\times$}
\expandafter\def\csname pv@ROBOTWIN_REACH_CODE\endcsname{618k}
\expandafter\def\csname pv@ROBOTWIN_REACH_LEVEL\endcsname{60.0\%}
\expandafter\def\csname pv@ROBOTWIN_REACH_REQ_CODE\endcsname{20}
\expandafter\def\csname pv@ROBOTWIN_REACH_REQ_RPENT\endcsname{40}
\expandafter\def\csname pv@ROBOTWIN_REACH_REQ_X\endcsname{2.0$\times$}
\expandafter\def\csname pv@ROBOTWIN_REACH_RPENT\endcsname{2.46M}
\expandafter\def\csname pv@ROBOTWIN_REACH_X\endcsname{4.0$\times$}
\expandafter\def\csname pv@ROBOTWIN_REQ1_CODE\endcsname{8.9}
\expandafter\def\csname pv@ROBOTWIN_REQ1_RPENT\endcsname{12.2}
\expandafter\def\csname pv@ROBOTWIN_REQ_CODE\endcsname{9}
\expandafter\def\csname pv@ROBOTWIN_REQ_RATIO_PT\endcsname{1.4$\times$}
\expandafter\def\csname pv@ROBOTWIN_REQ_RATIO_X2\endcsname{1.37$\times$}
\expandafter\def\csname pv@ROBOTWIN_REQ_RPENT\endcsname{12}
\expandafter\def\csname pv@ROBOTWIN_STEPS_CODE_X\endcsname{1.3$\times$}
\expandafter\def\csname pv@ROBOTWIN_SUCC_CODE\endcsname{173}
\expandafter\def\csname pv@ROBOTWIN_SUCC_RPENT\endcsname{150}
\expandafter\def\csname pv@ROBOTWIN_TASKS\endcsname{50}
\expandafter\def\csname pv@ROBOTWIN_TASKS_PHRASE\endcsname{all 50 RoboTwin 2.0 dual-arm tasks}
\expandafter\def\csname pv@ROBOTWIN_TPR_RATIO_PT\endcsname{1.2$\times$}
\expandafter\def\csname pv@ROBOTWIN_TPR_RATIO_X2\endcsname{1.23$\times$}
\expandafter\def\csname pv@ROBOTWIN_TTS_CODE\endcsname{90k}
\expandafter\def\csname pv@ROBOTWIN_TTS_DEC_CODE\endcsname{4}
\expandafter\def\csname pv@ROBOTWIN_TTS_DEC_RPENT\endcsname{7}
\expandafter\def\csname pv@ROBOTWIN_TTS_RPENT\endcsname{154k}
\expandafter\def\csname pv@ROBOTWIN_USD_CODE\endcsname{\$0.66}
\expandafter\def\csname pv@ROBOTWIN_USD_RPENT\endcsname{\$1.00}
\expandafter\def\csname pv@SHOW_SHARE\endcsname{84\%}
\expandafter\def\csname pv@SINGLE_STEP_ROBOTWIN\endcsname{54\%}
\expandafter\def\csname pv@SINGLE_STEP_SHARE\endcsname{35\%}
\expandafter\def\csname pv@SR_REL_RANGE\endcsname{10--15\%}
\expandafter\def\csname pv@STEPS_CODE_MAX\endcsname{1.3$\times$}
\expandafter\def\csname pv@STRETCH_CALLS_CODE\endcsname{2}
\expandafter\def\csname pv@STRETCH_CALLS_RPENT\endcsname{6}
\expandafter\def\csname pv@STRETCH_IMAGES_CODE\endcsname{1}
\expandafter\def\csname pv@STRETCH_IMAGES_RPENT\endcsname{12}
\expandafter\def\csname pv@STRETCH_TOK_CODE\endcsname{60k}
\expandafter\def\csname pv@STRETCH_TOK_RPENT\endcsname{380k}
\expandafter\def\csname pv@STRETCH_TOK_X\endcsname{6.3$\times$}
\expandafter\def\csname pv@TOKENS_SAVED_RANGE\endcsname{35--78\%}
\expandafter\def\csname pv@TOKF_RANGE\endcsname{1.5--4.5$\times$}
\expandafter\def\csname pv@TOOL_LLM_CALLS\endcsname{18,585}
\expandafter\def\csname pv@TOOL_ONE_SHARE\endcsname{89\%}
\expandafter\def\csname pv@TOOL_ONLY_N\endcsname{36}
\expandafter\def\csname pv@TOTAL_ABLATION_EPISODES\endcsname{3,200}
\expandafter\def\csname pv@TOTAL_BOTH\endcsname{406}
\expandafter\def\csname pv@TOTAL_MAIN_CELLS\endcsname{700}
\expandafter\def\csname pv@TOTAL_MAIN_EPISODES\endcsname{1,400}
\expandafter\def\csname pv@TOTAL_TASKS\endcsname{140}
\expandafter\def\csname pv@TWO_ACT_SHARE\endcsname{45\%}
\makeatother

